Hodge de Rham theory and analytic torsion for spaces with horn type singularities

We study the global analytic properties of a space $X$ with a horn type singularity. In particular, we introduce some de Rham complex of square integrable forms and we describe its homology and the spectral properties of the associated Hodge Laplace operator. All this is applied to produce a suitable description of the analytic torsion of $X$ and to prove an extension of the Cheeger M\"{u}ller theorem.

==> III1.2.tex <==




\subsection{The formal Hodge-Laplace operator near the singularity}\label{hodge} 
For a differentiable manifold $X$, and an orthogonal representation $\rho:\pi_1(X)\to O(V)$, we denote by $\Omega^{q}(X,E_\rho)$ the space of smooth sections of forms on $X$, with values in the associated vector bundle $E_\rho=V\otimes_\rho \widetilde X$, $\Gamma(X,\Lambda^{(q)}T^* E_\rho)$. 

We will now introduce a local description of the Hodge Laplace operator on forms near the singularity. Since we have seen that near the singularity any representation restricts to the trivial one, we will omit explicit reference to the bundle in the notation in this section.

Let $\star$, $d$, $d^\dagger$ and $\Delta$ denote the Hodge star, the exterior derivative, its dual and  Hodge-Laplace operator on $\ZZ$ induced by the metric $\g$. In this section we give the explicit form of these formal operators on $\ZZ$. It is clear that exactly the same analysis works replacing $\ZZ$ by $\CC$, and so we do to shorten notation. 


By separation of variables, it is clear that for any $\omega\in \Omega^{q}(\CC)$ we can write
\[
\omega(x,y)=f_1(x)\tilde\omega_1(y)+f_2(x)dx\wedge \tilde\omega_2(y),
\]
with smooth functions $f_1,f_2 \in C^{\infty}((0,l+\iota))$, and  forms, $\tilde\omega_1\in \Omega^{q}(W)$ and $\tilde\omega_2 \in \Omega^{q-1}(W)$. In other words, there is an identification of the spaces
\[
\Omega^{q}(\CC)=\CC^\infty\left((0,l+\iota), \Omega^q(W)\times \Omega^{q-1}(W)\right)
=\CC^\infty((0,l+\iota))\otimes  \left(\Omega^q(W)\times \Omega^{q-1}(W)\right).
\]






We perform some simplifications. Let $\al_q=q+\frac{1}{2}(1-m)$, and
\[
\omega=f_1\tilde\omega_1+f_2 dx\wedge \tilde\omega_2,
\]
then,
\begin{align*}
\star \omega=&
h^{1-2\al_{q-1}} f_2\tilde\star \tilde\omega_2+(-1)^q h^{1-2\al_{q}} f_1 
dx\wedge\tilde\star \tilde\omega_1,\\
d\omega  =&f_1 \tilde d\tilde\omega_1 + d x\wedge\left(  
f'_1 \tilde\omega_1 - f_2  \tilde \d\tilde\omega_2\right),\\
d^{\dag} \omega =& (-1)^{(m+1)q+(m+1)+1}\star d \star\omega\\
=&-h^{2\al_{q-1}-1} (h^{1-2\al_{q-1}}f_2)'\tilde\omega_2 + 
h^{-2}f_1 \tilde d^{\dag} \tilde\omega_1  - h^{-2}f_2dx \wedge \tilde d^{\dag} \tilde\omega_2,
\end{align*}
and
\begin{align*}
\Delta^{(q)}\omega=&(\FF_1^q f_1)\t\omega_1
-2\frac{h'}{h}f_2 \t d\t\omega_2
+(\FF_2^{q}) f_2 dx \wedge \t\omega_2
-2\frac{h'}{h^3}f_1 dx\wedge\t d^\da\t\omega_1.
\end{align*}
where
\begin{align*}
\FF_1^q f&=-h^{2\al_q-1}\left(h^{1-2\al_q}f'\right)' +\frac{\t\Delta^{(q)}}{h^2} f
=-f''-(1-2\al_q)\frac{h'}{h}f'+\frac{\t\Delta^{(q)}}{h^2} f,\\
\FF_2^{q}&=\FF_1^{q-1}-(1-2\al_{q-1})\left(\frac{h'}{h}\right)' .
\end{align*}


We proceed now to "diagonalise"  the formal Hodge Laplace operator. Let $\t\la$ be an eigenvalue of the Hodge Laplace operator on the section: $\t\Delta^{(q)} \t\om=\t\la\t\om$. Then, we have the Hodge decomposition of the space of forms on the section
\beq\label{dd1}
\Omega^q(W)=\bigoplus_{\t\la=0} \t\E^{(q)}_{\t\la},
\eeq
with the convention that $\t\E^{(q)}_{0}=\H^q(W)$, $\t\E^{(q)}_{\t\la>0}=\t\E^{(q)}_{\t\la,{\rm cex}}\oplus \t\E^{(q)}_{\t\la,{\rm ex}}$, and 
\begin{align*}
\H^q(W)&=\left\{\tilde\omega\in \Omega^{(q)}(W)~|~\tilde\Delta^{(q)}\tilde\omega=0\right\},\\
\tilde\E^{(q)}_{\tilde\la,{\rm ex}}&=\left\{\tilde\omega\in\Omega^{q}(W)~|~\tilde\Delta^{(q)}\tilde\omega=\tilde 
\lambda\tilde\omega, \, \tilde\omega=\tilde d\tilde\alpha\right\},\\
\tilde\E^{(q)}_{\tilde\la,{\rm cex}}&=\left\{\tilde\omega\in\Omega^{q}(W)~|~\tilde\Delta^{(q)}\tilde\omega=\tilde 
\lambda\tilde\omega, \, \tilde\omega=\tilde d^\dagger\tilde\alpha\right\}.
\end{align*}





This gives the direct sum decomposition
\begin{align*}
\Omega^q(\CC)=&\CC^\infty((0,l+\iota)) 
\otimes
\left( \bigoplus_{\t\la_1=0} \tilde\E^{(q)}_{\tilde\lambda_1}
\oplus \bigoplus_{\t\la_2=0} \tilde\E^{(q-1)}_{\tilde\lambda_2}\right),
\end{align*}
and 
\[
\Delta^{(q)}=\bigoplus_{  \t\la_1,\t\la_2=0}^\infty
\Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\t\E^{(q)}_{\tilde\lambda_{1}}\oplus  \tilde\E^{(q-1)}_{\tilde\lambda_{2}}\right)}.
\]



Let 
\[
\t A^q=\left\{\t\vv^{(q)}_{\la,j}\right\}=\left\{\tilde\varphi^{(q)}_{{\rm har},l}\right\}\cup \left\{\tilde\varphi^{(q)}_{\tilde\lambda,{\rm cex},j}\right\}\cup\left\{\tilde\varphi^{(q)}_{\tilde\lambda,{\rm ex},k}\right\},
\]
be an orthonormal bases of $\t\E_{\t\la}^{(q)}$, i.e. $\Omega^q(W)=\langle \t A_{\t\la}^q\rangle$. Then, the operator $\Delta^{(q)}$ decomposes as
\beq\label{decomp}
\Delta^{(q)}=\bigoplus_{  n_1,n_2=0}^\infty \Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\t\E^{(q)}_{\tilde\lambda_{1}}\oplus  \tilde\E^{(q-1)}_{\tilde\lambda_{2}}\right)},
\eeq
with
\[
\Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\t\E^{(q)}_{\tilde\lambda_{1}}\oplus  \tilde\E^{(q-1)}_{\tilde\lambda_{2}}\right)}=\bigoplus_{\t\la_1,\t\la_2}  \bigoplus_{j_1,j_2} \Delta^{(q)}_{\t\la_1,j_1,\t\la_2,j_2},
\]
where
\[
\Delta^{(q)}_{\t\la_1,j_1,\t\la_2,j_2}
=\Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\langle\t\vv^{(q)}_{\t\la_1,j_1}\rangle\oplus \langle\t\vv_{\t\la_2,j_2}\rangle\right)}
=\left(\begin{matrix} \tilde\vv^{(q)}_{\t\la_1,j_1} \FF^q_{1,\t\la_1}& -2\frac{h'}{h} \tilde \d\tilde\vv^{(q-1)}_{\t\la_2,j_2}\\
 -2\frac{h'}{h^3} \tilde \d^\da \t\vv^{(q)}_{\t\la_1,j_1}& \tilde\vv^{(q-1)}_{\t\la_2,j_2}\FF^{q}_{2,\t\la_2}\end{matrix}\right),
\]
acts on the space $C^\infty ((0,l+\iota),\R^2)$, and
\beq\label{F}
\begin{aligned}
\FF^q_{1,\t\la} f&=-h^{2\al_q-1}\left(h^{1-2\al_q}f'\right)' +\frac{\t\la}{h^2} f
=-f''-(1-2\al_q)\frac{h'}{h}f'+\frac{\t\la}{h^2} f,\\
\FF_{2,\t\la}^{q}&=\FF_{1,\t\la}^{q-1}-(1-2\al_{q-1})\left(\frac{h'}{h}\right)'.
\end{aligned}
\eeq
 


\begin{lem}\label{eigenforms} Let $\t\la\not= 0$ be an eigenvalue of $\t\Delta^{(q)}$,  with associated eigenspace $\tilde\E^{(q)}_{\t\la}=\tilde\E^{(q)}_{\t\la,{\rm cex}}\oplus \tilde\E^{(q)}_{\t\la,{\rm ex}}$. Let $\left\{\t\vv^{(q)}_{{\rm har},l}, \tilde\varphi_{\t\la,{\rm cex},j}^{(q)},\tilde\varphi_{\la,{\rm ex},k}^{(q-1)}\right\}$ be an orthonormal  basis 
of $\Omega^q(W)$ consisting of harmonic forms,   coexact and exact eigenforms associated to $\t\la$. 
%Let $J_\nu$ be the Bessel function of index $\nu$. Define 
%\begin{align*}
%\alpha_q &=\frac{1}{2}(1+2q-m), &\mu_{q,n} &= \sqrt{\lambda_{q,n}+\alpha_q^2}.
%\end{align*}
%and assume that $\al_q=q+\frac{1}{2}(1-m)$ is not an half integer. 
Then, the solutions of the equation $\Delta^{(q)} \omega=\lambda \omega$, 
with $\lambda\not=0$, are  of the following six types:
\[
\psi^{(q)}_{E}(x,\la)=f \t\vv^{(q)}_{{\rm har}},
\]
where $f$ is a solution of the equation $\FF^q_{1,0} f=\la f$;
\[
\psi^{(q)}_{I,\t\la}(x,\la)=f \t\vv^{(q)}_{\t\la,{\rm cex}},
\]
where $f$ is a solution of the equation $\FF^q_{1, \t\la} f=\la f$, $\t\la\not=0$;
\[
\psi^{(q)}_{O}(x,\la)=f dx\wedge\t \vv^{(q-1)}_{{\rm har}},
\]
where $f$ is a solution of the equation $\FF^{q}_{2,0} f=\la f$;
\[
\psi^{(q)}_{IV,\t\la}(x,\la)=f  dx \wedge\t\vv^{(q)}_{\t\la,{\rm ex}},
\]
where $f$ is a solution of the equation $\FF^{q}_{2,\t\la} f=\la f$, $\t\la\not=0$;
\[
\psi_{II,\t\la}^{(q)}=f \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}}+f'  dx\wedge \tilde\vv^{(q-1)}_{\t\la, {\rm cex}}
\]
where $f$ is a solution of $\FF^{q-1}_{1,\t\la} f=\la f$, $\t\la\not=0$; 
\[
\psi_{III,\t\la}^{(q)}
=-h^{2\al_q-1}\left(h^{1-\al_q}f\right)' \t\vv^{(q)}_{\t\la, \rm ex}-\frac{f}{h^2} dx\wedge \t d^\da \t\vv^{(q)}_{\t\la, \rm ex},
\]
where $f$ a solution of the equation $\FF^{q+1}_{2,\t\la}f=\la f$, with $\t\la\not=0$. 
\end{lem}


\begin{proof} Write $\om\in \CC^\infty((0,l+\iota))\otimes\left(\langle\t\vv^{(q)}_{\t\la_1,j_1}\rangle\oplus \langle\t\vv_{\t\la_2,j_2}\rangle\right)$ as
\[
\om=f_1 \tilde\vv^{(q)}_{\t\la_1,j_1}+f_2 dx\wedge \tilde\vv^{(q-1)}_{\t\la_2,j_2}.
\]

Then, using the decomposition in equation (\ref{decomp}), the solutions of the equation 
\[
\Delta^{(q)} \om=\la\om,
\]
are given by the union of the solutions of the  equations
\begin{align*}
\Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\t\E^{(q)}_{\tilde\lambda_{1}}\oplus  \tilde\E^{(q-1)}_{\tilde\lambda_{2}}\right)}\om&=\la\om,
\end{align*}
that are given by the linear combination of the solutions of the equations
\begin{align*}
\Delta^{(q)}|_{\CC^\infty((0,l+\iota))\otimes\left(\langle\t\vv^{(q)}_{\t\la_1,j_1}\rangle\oplus \langle\t\vv_{\t\la_2,j_2}\rangle\right)}\left( \begin{matrix}f_1\\f_2\end{matrix}\right)&=\la (\tilde\vv^{(q)}_{\t\la_1,j_1}\ss \tilde\vv^{(q-1)}_{\t\la_2,j_2}) \left( \begin{matrix}f_1\\ f_2\end{matrix}\right)\\
\left(\begin{matrix} \tilde\vv^{(q)}_{\t\la_1,j_1} \FF^q_{1,\t\la_1}& -2\frac{h'}{h} \tilde \d\tilde\vv^{(q-1)}_{\t\la_2,j_2}\\
-2\frac{h'}{h^3} \tilde \d^\da \t\vv^{(q)}_{\t\la_1,j_1}& \tilde\vv^{(q-1)}_{\t\la_2,j_2}\FF^{q}_{2,\t\la_2}\end{matrix}\right)
\left( \begin{matrix}f_1\\f_2\end{matrix}\right)
&=\la \left( \begin{matrix}f_1\tilde\vv^{(q)}_{\t\la_1,j_1}\\f_2  \tilde\vv^{(q-1)}_{\t\la_2,j_2}\end{matrix}\right).
\end{align*}


Each of these equations has solution only if either 1) both the following two conditions are satisfied:  a) either $f_2=0$ or $\t d\t\vv^{(q-1)}_{\t\la_2,j_2}=0$, b) $f_1=0$ or $\t d^\da\t\vv^{(q)}_{\t\la_1,j_1}=0$, or 
2)  $\t\vv^{(q)}_{\t\la_1,j_1}= \t d \t\vv^{(q-1)}_{\t\la_2,j_2}$. %, or $\t d^\da \t\vv^{(q)}_{\t\la_1,j_1}=  \t\vv^{(q-1)}_{\t\la_2,j_2}$.

We will omit the indices $j_1, j_2$ in the final formula for the solutions.

\noindent 1) If $f_2=0$ and $\t d^\da\vv^{(q)}_{\t\la_1,j_1}=0$, then either $\t\vv^{(q)}_{\t\la_1,j_1}$ is harmonic, and we have the solution
\[
\psi^{(q)}_{E}(x,\la)=f_1 \t\vv^{(q)}_{{\rm har}},
\]
where $f_1$ is a solution of the equation
\[
\FF^q_{1,0} f_1=\la f_1,
\]
or $\t\vv^{(q)}_{\t\la_1,j_1}$ is coexact, and we have the solution
\[
\psi^{(q)}_{I,\t\la}(x,\la)=f_1 \t\vv^{(q)}_{\t\la,{\rm cex}},
\]
where $f_1$ is a solution of the equation
\[
\FF^q_{1,\t\la} f_1=\la f_1.
\]

If $f_1=0$ and $\t d \t\vv^{(q-1)}_{\t\la_2,j_2}=0$, then either $\t\vv^{(q-1)}_{\t\la_2,j_2}$ is harmonic, and we have the solution
\[
\psi^{(q)}_{O}(x,\la)=f_2 dx\wedge\t \vv^{(q-1)}_{{\rm har}},
\]
where $f_2$ is a solution of the equation
\[
\FF^{q}_{2,0} f_2=\la f_2,
\]
or $\t\vv^{(q-1)}_{\t\la_2,j_2}$ is exact, and we have the solution
\[
\psi^{(q)}_{IV,\t\la}(x,\la)=f_2  dx \wedge\t\vv^{(q)}_{\t\la,{\rm ex}},
\]
where $f_2$ is a solution of the equation
\[
\FF^{q}_{2,\t\la} f_2=\la f_2.
\]

\noindent 2) If $\t\vv^{(q)}_{\t\la_1,j_1}=\t d \t\vv^{(q-1)}_{\t\la_2,j_2}$, and $\t\la_1=\t\la_2=\t\la$, then $\t\vv^{(q)}_{\t\la_1,j_1}$ is exact and $\t\vv^{(q-1)}_{\t\la_2,j_2}$ coexact, $\t\la_1=\t\la_2$ (since $\Delta d=d\Delta$), and then
\[
\om=f_1 \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}}+f_2  dx\wedge \tilde\vv^{(q-1)}_{\t\la, {\rm cex}},
\]
also observe that
\[
\t d^\da \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}}=\t \Delta  \t\vv^{(q-1)}_{\t\la, {\rm cex}}=\t\la  \t\vv^{(q-1)}_{\t\la, {\rm cex}}.
\]

Thus, we obtain the equations
\[
\left\{
\begin{array}{l} -f_1''-(1-2\al_q)\frac{h'}{h}f_1'-2\frac{h'}{h}f_2 +\frac{\t\la}{h^2} f_1=\la f_1,\\
-f_2''-(1-2\al_{q-1})\frac{h'}{h}f_2'-(1-2\al_{q-1})\left(\frac{h'}{h}\right)'f_2-2\t\la \frac{h'}{h^3}f_1 +\frac{\t\la}{h^2} f_2=\la f_2.
\end{array}
\right.
\]
 
 
A solution is given by $f_2=f_1'$. For substitution in the first equation gives
\[
-f_1''-(1-2\al_{q-1})\frac{h'}{h}f_1'+\frac{\t\la}{h^2} f_1 =\la f_1,
\]
that differentiated gives
\[
-f_1'''-(1-2\al_{q-1})\frac{h'}{h}f_1''-(1-2\al_{q-1})\left(\frac{h'}{h}\right)'f'_1-2\t\la\frac{h'}{h^3}f_1 +\frac{\t\la}{h^2} f'_1=\la f_1',
\]
that is precisely the second equation of the system with $f_2=f_1'$.  This solution gives the form
\[
\psi_{II,\t\la}^{(q)}=f_1 \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}}+f'_1  dx\wedge \tilde\vv^{(q-1)}_{\t\la, {\rm cex}}
=d(f_1 \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}})=d \psi_{I,\t\la}^{(q-1)},
\]
where $f_1$ is a solution of
\[
\FF^{q-1}_{1,\t\la} f_1=\la f_1.
\]


This solution comes from the commutativity $\Delta d=d \Delta$. Thus, a second solution will come from the commutativity 
$\Delta d^\da=d^\da \Delta$, and will be of the type 
\[
\psi_{III,\t\la}^{(q)}=d^\da \psi_{IV,\t\la}^{(q+1)}=d^\da \left( f_2 dx \wedge \t\vv^{(q)}_{\t\la,\rm ex}\right)
=-h^{2\al_q-1}\left(h^{1-\al_q}f_2\right)' \t\vv^{(q)}_{\t\la, \rm ex}-\frac{f_2}{h^2} dx\wedge \t d^\da \t\vv^{(q)}_{\t\la, \rm ex},
\]
with $f_2$ a solution of the equation
\[
\FF^{q+1}_{2,\t\la}f_2=\la f_2.
\]

In fact, taking the vector
\[
\left( \begin{matrix}f_1\\ f_2\end{matrix}\right)
=\left( \begin{matrix}-h^{2\al_q-1}\left(h^{1-\al_q}f_2\right)'\\ -\frac{f_2}{h^2}\end{matrix}\right),
\]
after some calculation, we verify that it satisfy the equation 
\begin{align*}
\left(\begin{matrix} \t\vv^{(q)}_{\t\la, \rm ex} \FF^q_{1,\t\la_1}& -2\frac{h'}{h} \t\la \t\vv^{(q)}_{\t\la, \rm ex}\\
-2\frac{h'}{h^3} \tilde \d^\da \t\vv^{(q)}_{\t\la, \rm ex}& \t d^\da\t\vv^{(q)}_{\t\la, \rm ex}\FF^{q}_{2,\t\la_2}\end{matrix}\right)
\left( \begin{matrix}f_1\\f_2\end{matrix}\right)
&=\la \left( \begin{matrix}f_1\t\vv^{(q)}_{\t\la, \rm ex}\\f_2 \t d^\da\t\vv^{(q)}_{\t\la, \rm ex}\end{matrix}\right).
\end{align*}

The easiest way to see that is to substitute in the second equation, do the calculation that will transform the second equation in the equation $\FF^{q+1}_{2,\t\la}f_2=\la f_2$, and then differentiate, do the calculation and arrive to the first equation of the system. \end{proof}

\begin{rem}\label{rem1.1} Observe that:
\begin{align*}
d \psi_{O,\t\la} & =d \psi_{II,\t\la}= d \psi_{IV,\t\la}=0,\\
d \psi_{E,\t\la,j} &=  \psi_{O,\t\la,k\not=j},\\
d \psi_{I,\t\la,j} &=  \psi_{II,\t\la,k\not=j},\\
d \psi_{III,\t\la,j} &=  \psi_{IV,\t\la,k\not=j},\\
d^\da \psi_{E,\t\la} & =d^\da \psi_{I,\t\la}= d^\da \psi_{II,\t\la}=0,\\
d^\da \psi_{O,\t\la,j} &=  \psi_{E,\t\la,k\not=j},\\
d^\da \psi_{II,\t\la,j} &=  \psi_{I,\t\la,k\not=j},\\
d^\da \psi_{IV,\t\la,j} &=  \psi_{III,\t\la,k\not=j}.
\end{align*}
\end{rem}

\begin{lem}\label{harmonics} Let $\t\la\not= 0$ be an eigenvalue of $\t\Delta^{(q)}$,  with associated eigenspace $\tilde\E^{(q)}_{\t\la}=\tilde\E^{(q)}_{\t\la,{\rm cex}}\oplus \tilde\E^{(q)}_{\t\la,{\rm ex}}$. Let $\left\{\t\vv^{(q)}_{{\rm har},l}, \tilde\varphi_{\t\la,{\rm cex},j}^{(q)},\tilde\varphi_{\la,{\rm ex},k}^{(q-1)}\right\}$ be an orthonormal  basis 
of $\Omega^q(W)$ consisting of harmonic forms,   coexact and exact eigenforms associated to $\t\la$. 
%Let $J_\nu$ be the Bessel function of index $\nu$. Define 
%\begin{align*}
%\alpha_q &=\frac{1}{2}(1+2q-m), &\mu_{q,n} &= \sqrt{\lambda_{q,n}+\alpha_q^2}.
%\end{align*}
%and assume that $\al_q=q+\frac{1}{2}(1-m)$ is not an half integer. 
Then, the solutions of the equation $\Delta^{(q)} \omega=0$, 
with $\lambda\not=0$, are  of the following five types:
\[
\psi^{(q)}_{E}(x,\la)=f \t\vv^{(q)}_{{\rm har}},
\]
where $f$ is a solution of the equation $\FF^q_{1,0} f=0$;
\[
\psi^{(q)}_{I,\t\la}(x,\la)=f \t\vv^{(q)}_{\t\la,{\rm cex}},
\]
where $f$ is a solution of the equation $\FF^q_{1, \t\la} f=0$, $\t\la\not=0$;
\[
\psi^{(q)}_{O}(x,\la)=f dx\wedge\t \vv^{(q-1)}_{{\rm har}},
\]
where $f$ is a solution of the equation $\FF^{q}_{2,0} f=0$;
\[
\psi^{(q)}_{IV,\t\la}(x,\la)=f  dx \wedge\t\vv^{(q)}_{\t\la,{\rm ex}},
\]
where $f$ is a solution of the equation $\FF^{q}_{2,\t\la} f=0$, $\t\la\not=0$;
\[
\psi_{II,\t\la}^{(q)}=f \t d \t\vv^{(q-1)}_{\t\la, {\rm cex}}+f'  dx\wedge \tilde\vv^{(q-1)}_{\t\la, {\rm cex}}
\]
where $f$ is a solution of $\FF^{q-1}_{1,\t\la} f=0$, $\t\la\not=0$. 
\end{lem}
\begin{proof} The proof is the same as that of Lemma \ref{eigenforms}. It remains to show that each harmonics of type II is also of type III. Here is a proof. Fix an eigenvalue $\t\la$ and let $\vv$ a coexact eigenform with eigenvalue $\t\la$. Take a form of type I
\[
\vv^{(q-1)}=f\t\vv,
\]
with $\FF^{q-1}_{1,\t\la}f=0$, and a form of type IV
\[
\be^{(q+1)}=g dx \wedge \t d \t\be,
\]
with $\FF^{q+1}_{2,\t\la}g=0$. Recall that
\[
d\vv=f\t d\t\vv+f' dx\wedge\t\vv,
\]
and 
\[
d^\da \be=-h^{2\al_{q}-1} (h^{1-2\al_{q}}g)'\t \be - \frac{g}{h^2}dx \wedge \tilde d^{\dag} \tilde\be.
\]

We show that if  $\t\be=-\frac{1}{\t\la}\t d\vv$, and $g=h^2 f$, then
\[
d\vv=d^\da\be.
\]

For, we compute 
\[
d^\da \be=\frac{1}{\t\la}h^{2\al_{q}-1} (h^{3-2\al_{q}}f')'\t d\t \vv +f'dx \wedge \t\vv,
\]
where we used the fact that $\t d^\da \t d \t\vv=\t\la\t\vv$. Now it is immediate to see that
\[
\frac{1}{\t\la}h^{2\al_{q}-1} (h^{3-2\al_{q}}f')'=f,
\]
since this is exactly the equation $\FF^{q-1}_{1,\t\la}f=0$, verified by $f$. A little bit more work is necessary in order to prove that $g=h^2 f'$ satisfies the equation $\FF^{q+1}_{2,\t\la}g=0$, as requested. In order to see that develop the equation
\[
\FF^{q+1}_{2,\t\la}(h^2 f')=0.
\]

We obtain the equation
\[
-f'''-(3-2\al_q)\frac{h'}{h}f''-(3-2\al_q)\left(\frac{h'}{h}\right)' f'+\frac{\t\la}{h^2} f'-2\t\la \frac{h'}{h^3}f=0,
\]
while differentiation of the equation $\FF^{q-1}_{1,\t\la}f=0$, gives the equation
\[
-f'''-(3-2\al_q)\frac{h'}{h}f''-(3-2\al_q)\left(\frac{h'}{h}\right)' f'+\frac{\t\la}{h^2} f'+2\frac{h'}{h}\left(-f''-(3-2\al_q)\frac{h'}{h}f'\right)=0,
\]
that exploiting again $\FF^{q-1}_{1,\t\la}f=0$ reduces to the previous one. 
\end{proof}




\subsection{Hilbert space and square integrability of the solutions of the eigenvalues equation}

Let $(X,g_X)$, where $X=\ZZ\cup_W Y$, be a space with horn singularities as defined in Section \ref{horn}. Let $\pi$ be either $\pi_1(X)$ or $\pi_1(Y)$, $\rho:\pi \to O(V)$ a (real) orthogonal representation, and $E_\rho=V\otimes_\rho \widetilde X$ the associated vector bundle, again as defined in Section \ref{horn}.  
We will study the Hodge Laplace operator of $(X,g_X)$ in the Hilbert space $L^2(X)$, the space of the sections 
$\om,\vv\in \Gamma(X,E_\rho)$, with finite norm with respect to the inner product
\[
\langle \om,\vv\rangle=\int_{X} \om\wedge\star \vv=\int_{\ZZ} \om\wedge\star \vv+\int_{Y} \om\wedge\star \vv.
\]

Restricting on $\CC$, $\om$ and $\vv$  read 
\begin{align*}
\om&=f_1\tilde\omega_1+f_2 dx\wedge \tilde\omega_2, &
\vv&=g_1\tilde\vv_1+g_2 dx\wedge \tilde\vv_2,
\end{align*}
and a direct calculation exploiting the formula for the hodge star gives
\[
\langle \om,\vv\rangle_\CC=\int_0^l h^{1-2\al_{q}} f_1 g_1 dx \langle \t\om_1,\t\vv_1\rangle_W
+\int_0^l h^{1-2\al_{q-1}} f_2 g_2 dx \langle \t\om_2,\t\vv_2\rangle_W,
\]
where
\[
\langle \t\om,\t\vv\rangle_W=\int_W \t\om\wedge \t\star\t\vv.
\]






\subsection{Concrete operator}
--------------------



Since the differential defines a bijection %(an isometry if normalised by $\frac{1}{\la}$)
\begin{align*}
\tilde \d:&\tilde\E^{(q)}_{\tilde\lambda,{\rm cex}}\to \tilde\E^{(q+1)}_{\tilde\lambda, {\rm ex}},&
\tilde \d:&\tilde\varphi\mapsto \tilde d\tilde\varphi,
\end{align*}
whose inverse is $\tilde \d^\da$, we may rewrite
\beq\label{bas1}
\t A_{\t\la}^q=\left\{\tilde\varphi_{{\rm har},l}^{(q)}\right\}_l\cup\bigcup_{n=1}^\infty\left\{\tilde\varphi_{\tilde\lambda_{q,n},{\rm cex},j}^{(q)},\t d\tilde\varphi_{\tilde\lambda_{q,n},{\rm cex},k}^{(q-1)}\right\}_{j,k}.
\eeq












\textcolor{red}{dopo}
Thus, the relevant formal operators appearing in the Laplace operator are
\begin{align*}
\FF_q f&=-h^{2\al_q-1}\left(h^{1-2\al_q}f'\right)' +\frac{\t\Delta^{(q)}}{h^2} f
=-f''-(1-2\al_q)\frac{h'}{h}f'+\frac{\t\Delta^{(q)}}{h^2} f.
\end{align*}


This is a  formal second order Sturm Liouville operator, that in the usual notation \cite[?]{Zet} reads
\[
\lf y=\frac{1}{w}(-(py')'+qy)=-\frac{p}{w}y''-\frac{p'}{w}y'+\frac{q}{w}y,
\]
with 
\begin{align*}
p&=w=h^{1-2\al_q},&q&=\frac{\t\Delta^{(q)}}{h^2} h^{1-2\al_q}.
\end{align*}








The change of variable
\begin{align*}
f_1&=h^{\al_q-\frac{1}{2}} u_1,\\
f_2&=h^{\al_q-\frac{1}{2}} u_2,
\end{align*}



\appendix
%\input{appendices.1}






\bibliographystyle{plain}
\bibliography{HarSprBibliography.bib}




\end{document}





==> domains_of_Laplacian.tex <==



\begin{prop}\label{domLapminmax} The domain of the absolute and relative  Hodge Laplace operators is as follows. Let $\al$ be a form that locally reads $\al|_{\CF}=a_1\t\al_1+dx\wedge a_2\t\al_2$. Then,  
\begin{enumerate}

\item $\DS(\Delta^{(q)}_{\d})$ is the set:
\begin{enumerate}

\item $\al\in \DS(\d_{\rm max}^{(q)})\cap  \DS(\dr_{\rm max}^{(q)})$, and $D \al\in \DS(\dr_{\rm max}^{(q+1)})$ and $\DD \al\in \DS(\d_{\rm max}^{(q-1)})$,

\item %at $\b X$:
$
\left\{\begin{array}{l} bv_{\rm rel}(\b X)(\al)=0,\\ bv_{\rm rel}(\b X)(\DD\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_1(l)=0,\\ (h^{1-2\al_{q-1}}a_2)^I(l)=0,\end{array}\right.
$

\item %at $x_0$:

$\left\{\begin{array}{l} bv^{(q)}_{\rm rel}(x_0)(\al)=0,\\ bv^{(q-1)}_{\rm rel}(x_0)(\DD\al)=0.\end{array}\right. 
$
\end{enumerate}

\item $\DS(\Delta^{(q)}_{\dr})$ is the set:
\begin{enumerate}

\item $\al\in \DS(\d_{\rm max}^{(q)})\cap  \DS(\dr_{\rm max}^{(q)})$, and $D \al\in \DS(\dr_{\rm max}^{(q+1)})$ and $\DD \al\in \DS(\d_{\rm max}^{(q-1)})$,

\item %at $\b X$:
$
\left\{\begin{array}{l} bv_{\rm abs}(\b X)(\al)=0,\\ bv_{\rm abs}(\b X)(\DD\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_1(l)=0,\\ (h^{1-2\al_{q-1}}a_2)^I(l)=0,\end{array}\right.
$

\item %at $x_0$:

$\left\{\begin{array}{l} bv^{(q)}_{\rm abs}(x_0)(\al)=0,\\ bv^{(q-1)}_{\rm abs}(x_0)(\DD\al)=0.\end{array}\right. 
$
\end{enumerate}
\end{enumerate}
\end{prop}


\begin{prop}\label{domLap} The domain of the intersection Hodge Laplace operators is as follows. Let $\al$ be a form that locally reads $\al|_{\CF}=a_1\t\al_1+dx\wedge a_2\t\al_2$. Then,  if $m=2p-1$ 
\begin{enumerate}

\item $\DS(\Delta^{(q)}_{\dr, \pf,\rm abs})$ is the set:
\begin{enumerate}

\item $\al\in \DS(\d_{\rm max}^{(q)})\cap  \DS(\dr_{\rm max}^{(q)})$, and $D \al\in \DS(\dr_{\rm max}^{(q+1)})$ and $\DD \al\in \DS(\d_{\rm max}^{(q-1)})$,

\item %at $\b X$:
$
\left\{\begin{array}{l} bv_{\rm abs}(\b X)(\al)=0,\\ bv_{\rm abs}(\b X)(D\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_2(l)=0,\\ a_1^I(l)=0,\end{array}\right.
$


\item %at $x_0$:
\begin{align*}
&\left\{\begin{array}{l} bv^{(q)}_{\rm rel}(x_0)(\al)=0,\\ bv^{(q-1)}_{\rm rel}(x_0)(\DD\al)=0,\end{array}\right. 0\leq q\leq p,\\
&\left\{\begin{array}{l} bv^{(p)}_{\rm rel}(x_0)(\DD\al)=0,\\ bv^{(p+2)}_{\rm abs}(x_0)(D\al)=0,\end{array}\right. q=p+1,\\
&\left\{\begin{array}{l} bv^{(q)}_{\rm abs}(x_0)(\al)=0,\\ bv^{(q+1)}_{\rm abs}(x_0)(D\al)=0,\end{array}\right. p+2\leq q\leq 2p-1.
\end{align*}

\end{enumerate}

\item $\D(\Delta^{(q)}_{\d, \pf, \rm rel})$ coincides with $\D(\Delta^{(q)}_{\dr, \pf, \rm abs})$ with condition (b) replaced by
\begin{enumerate}

\item[(b')] %at $\b X$:
$
\left\{\begin{array}{l} bv_{\rm rel}(\b X)(\al)=0,\\ bv_{\rm rel}(\b X)(\DD\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_1(l)=0,\\ (h^{1-2\al_{q-1}}a_2)^I(l)=0,\end{array}\right.
$

\end{enumerate}

\end{enumerate}

If $m=2p$, then $\DS(\Delta^{(q)}_{\d, \mf^c, \rm rel})=\DS(\Delta^{(q)}_{\dr, \mf^c, \rm abs})$ is the same as in the case $m=2p-1$, while
\begin{enumerate}

\item $\DS(\Delta^{(q)}_{\dr, \mf, \rm abs})$ is the following set:
\begin{enumerate}

\item $\al\in \DS(\d_{\rm max}^{(q)})\cap  \DS(\dr_{\rm max}^{(q)})$, and $D \al\in \DS(\dr_{\rm max}^{(q+1)})$ and $\DD \al\in \DS(\d_{\rm max}^{(q-1)})$,

\item %at $x=\b X$:
$
\left\{\begin{array}{l} bv_{\rm abs}(\b X)(\al)=0,\\ bv_{\rm abs}(\b X)(D\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_2(l)=0,\\ a_1^I(l)=0,\end{array}\right.
$


\item %at $x_0$:
\begin{align*}
&\left\{\begin{array}{l} bv^{(q)}_{\rm rel}(x_0)(\al)=0,\\ bv^{(q-1)}_{\rm rel}(x_0)(\DD\al)=0,\end{array}\right. 0\leq q\leq p-1,\\
&\left\{\begin{array}{l} bv^{(p-1)}_{\rm rel}(x_0)(\DD\al)=0,\\ bv^{(p+1)}_{\rm abs}(x_0)(D\al)=0,\end{array}\right. q=p,\\
&\left\{\begin{array}{l} bv^{(q)}_{\rm abs}(x_0)(\al)=0,\\ bv^{(q+1)}_{\rm abs}(x_0)(D\al)=0,\end{array}\right. p+1\leq q\leq 2p-1.
\end{align*}

\end{enumerate}

\item $\DS(\Delta^{(q)}_{\d, \mf, \rm rel})$ coincides with $\D(\Delta^{(q)}_{\dr, \mf, \rm abs})$ with condition (b) replaced by
\begin{enumerate}

\item[(b')] %at $\b X$:
$
\left\{\begin{array}{l} bv_{\rm rel}(\b X)(\al)=0,\\ bv_{\rm rel}(\b X)(\DD\al)=0,\end{array}\right.
%=\left\{\begin{array}{l} a_1(l)=0,\\ (h^{1-2\al_{q-1}}a_2)^I(l)=0,\end{array}\right.
$

\end{enumerate}

\end{enumerate}


\end{prop}



